Adversarial TableQA: Attention Supervision for Question Answering on Tables

The task of answering a question given a text passage has shown great developments on model performance thanks to community efforts in building useful datasets. Recently, there have been doubts whether such rapid progress has been based on truly understanding language. The same question has not been asked in the table question answering (TableQA) task, where we are tasked to answer a query given a table. We show that existing efforts, of using "answers" for both evaluation and supervision for TableQA, show deteriorating performances in adversarial settings of perturbations that do not affect the answer. This insight naturally motivates to develop new models that understand question and table more precisely. For this goal, we propose Neural Operator (NeOp), a multi-layer sequential network with attention supervision to answer the query given a table. NeOp uses multiple Selective Recurrent Units (SelRUs) to further help the interpretability of the answers of the model. Experiments show that the use of operand information to train the model significantly improves the performance and interpretability of TableQA models. NeOp outperforms all the previous models by a big margin.

==> acml18 <==
\begin{thebibliography}{32}
\providecommand{\natexlab}[1]{#1}
\providecommand{\url}[1]{\texttt{#1}}
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi: #1}\else
  \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi

\bibitem[Amplayo et~al.(2018{\natexlab{a}})Amplayo, Kim, Sung, and won
  Hwang]{Amplayo2018ColdStartAU}
Reinald~Kim Amplayo, Jihyeok Kim, Sua Sung, and Seung won Hwang.
\newblock Cold-start aware user and product attention for sentiment
  classification.
\newblock In \emph{ACL}, 2018{\natexlab{a}}.

\bibitem[Amplayo et~al.(2018{\natexlab{b}})Amplayo, Lee, Yeo, and won
  Hwang]{Amplayo2018TranslationsAA}
Reinald~Kim Amplayo, Kyungjae Lee, Jinyeong Yeo, and Seung won Hwang.
\newblock Translations as additional contexts for sentence classification.
\newblock In \emph{IJCAI}, 2018{\natexlab{b}}.

\bibitem[Amplayo et~al.(2018{\natexlab{c}})Amplayo, Lim, and won
  Hwang]{amplayo2017entity}
Reinald~Kim Amplayo, Seonjae Lim, and Seung won Hwang.
\newblock Entity commonsense representation for neural abstractive
  summarization.
\newblock In \emph{NAACL}, 2018{\natexlab{c}}.

\bibitem[Bahdanau et~al.(2014)Bahdanau, Cho, and Bengio]{bahdanau2014neural}
Dzmitry Bahdanau, Kyunghyun Cho, and Yoshua Bengio.
\newblock Neural machine translation by jointly learning to align and
  translate.
\newblock \emph{arXiv preprint arXiv:1409.0473}, 2014.

\bibitem[Berant et~al.(2013)Berant, Chou, Frostig, and
  Liang]{berant2013semantic}
Jonathan Berant, Andrew Chou, Roy Frostig, and Percy Liang.
\newblock Semantic parsing on freebase from question-answer pairs.
\newblock In \emph{Proceedings of the 2013 Conference on Empirical Methods in
  Natural Language Processing}, pages 1533--1544, 2013.

\bibitem[Chung et~al.(2014)Chung, Gulcehre, Cho, and
  Bengio]{chung2014empirical}
Junyoung Chung, Caglar Gulcehre, KyungHyun Cho, and Yoshua Bengio.
\newblock Empirical evaluation of gated recurrent neural networks on sequence
  modeling.
\newblock \emph{arXiv preprint arXiv:1412.3555}, 2014.

\bibitem[Cui et~al.(2017)Cui, Xiao, Wang, Song, Hwang, and Wang]{cui2017kbqa}
Wanyun Cui, Yanghua Xiao, Haixun Wang, Yangqiu Song, Seung-won Hwang, and Wei
  Wang.
\newblock Kbqa: learning question answering over qa corpora and knowledge
  bases.
\newblock \emph{Proceedings of the VLDB Endowment}, 10\penalty0 (5):\penalty0
  565--576, 2017.

\bibitem[Das et~al.(2017)Das, Agrawal, Zitnick, Parikh, and
  Batra]{das2017human}
Abhishek Das, Harsh Agrawal, Larry Zitnick, Devi Parikh, and Dhruv Batra.
\newblock Human attention in visual question answering: Do humans and deep
  networks look at the same regions?
\newblock \emph{Computer Vision and Image Understanding}, 163:\penalty0
  90--100, 2017.

\bibitem[Dong and Lapata(2016)]{dong2016language}
Li~Dong and Mirella Lapata.
\newblock Language to logical form with neural attention.
\newblock \emph{arXiv preprint arXiv:1601.01280}, 2016.

\bibitem[Glorot and Bengio(2010)]{glorot2010understanding}
Xavier Glorot and Yoshua Bengio.
\newblock Understanding the difficulty of training deep feedforward neural
  networks.
\newblock In \emph{Proceedings of the Thirteenth International Conference on
  Artificial Intelligence and Statistics}, pages 249--256, 2010.

\bibitem[Goldman et~al.(2017)Goldman, Latcinnik, Naveh, Globerson, and
  Berant]{goldman2017weakly}
Omer Goldman, Veronica Latcinnik, Udi Naveh, Amir Globerson, and Jonathan
  Berant.
\newblock Weakly-supervised semantic parsing with abstract examples.
\newblock \emph{arXiv preprint arXiv:1711.05240}, 2017.

\bibitem[Hinton et~al.(2012)Hinton, Srivastava, Krizhevsky, Sutskever, and
  Salakhutdinov]{hinton2012improving}
Geoffrey~E Hinton, Nitish Srivastava, Alex Krizhevsky, Ilya Sutskever, and
  Ruslan~R Salakhutdinov.
\newblock Improving neural networks by preventing co-adaptation of feature
  detectors.
\newblock \emph{arXiv preprint arXiv:1207.0580}, 2012.

\bibitem[Jia and Liang(2017)]{jia2017adversarial}
Robin Jia and Percy Liang.
\newblock Adversarial examples for evaluating reading comprehension systems.
\newblock \emph{arXiv preprint arXiv:1707.07328}, 2017.

\bibitem[Krishnamurthy and Kollar(2013)]{krishnamurthy2013jointly}
Jayant Krishnamurthy and Thomas Kollar.
\newblock Jointly learning to parse and perceive: Connecting natural language
  to the physical world.
\newblock \emph{Transactions of the Association for Computational Linguistics},
  1:\penalty0 193--206, 2013.

\bibitem[Kwiatkowski et~al.(2013)Kwiatkowski, Choi, Artzi, and
  Zettlemoyer]{kwiatkowski2013scaling}
Tom Kwiatkowski, Eunsol Choi, Yoav Artzi, and Luke Zettlemoyer.
\newblock Scaling semantic parsers with on-the-fly ontology matching.
\newblock In \emph{2013 Conference on Empirical Methods in Natural Language
  Processing, EMNLP 2013}. Association for Computational Linguistics (ACL),
  2013.

\bibitem[Liu et~al.(2017{\natexlab{a}})Liu, Mao, Sha, and
  Yuille]{liu2017attention}
Chenxi Liu, Junhua Mao, Fei Sha, and Alan~L Yuille.
\newblock Attention correctness in neural image captioning.
\newblock In \emph{AAAI}, pages 4176--4182, 2017{\natexlab{a}}.

\bibitem[Liu et~al.(2017{\natexlab{b}})Liu, Shen, Duh, and
  Gao]{liu2017stochastic}
Xiaodong Liu, Yelong Shen, Kevin Duh, and Jianfeng Gao.
\newblock Stochastic answer networks for machine reading comprehension.
\newblock \emph{arXiv preprint arXiv:1712.03556}, 2017{\natexlab{b}}.

\bibitem[Mi et~al.(2016)Mi, Wang, and Ittycheriah]{mi2016supervised}
Haitao Mi, Zhiguo Wang, and Abe Ittycheriah.
\newblock Supervised attentions for neural machine translation.
\newblock In \emph{Proceedings of the 2016 Conference on Empirical Methods in
  Natural Language Processing}, pages 2283--2288, 2016.

\bibitem[Min et~al.(2017)Min, Seo, and Hajishirzi]{min2017question}
Sewon Min, Minjoon Seo, and Hannaneh Hajishirzi.
\newblock Question answering through transfer learning from large fine-grained
  supervision data.
\newblock \emph{arXiv preprint arXiv:1702.02171}, 2017.

\bibitem[Neelakantan et~al.(2015)Neelakantan, Le, and
  Sutskever]{neelakantan2015neural}
Arvind Neelakantan, Quoc~V Le, and Ilya Sutskever.
\newblock Neural programmer: Inducing latent programs with gradient descent.
\newblock \emph{arXiv preprint arXiv:1511.04834}, 2015.

\bibitem[Neelakantan et~al.(2016)Neelakantan, Le, Abadi, McCallum, and
  Amodei]{neelakantan2016learning}
Arvind Neelakantan, Quoc~V Le, Martin Abadi, Andrew McCallum, and Dario Amodei.
\newblock Learning a natural language interface with neural programmer.
\newblock \emph{arXiv preprint arXiv:1611.08945}, 2016.

\bibitem[Pasupat and Liang(2015)]{pasupat2015compositional}
Panupong Pasupat and Percy Liang.
\newblock Compositional semantic parsing on semi-structured tables.
\newblock \emph{arXiv preprint arXiv:1508.00305}, 2015.

\bibitem[Rajpurkar et~al.(2016)Rajpurkar, Zhang, Lopyrev, and
  Liang]{rajpurkar2016squad}
Pranav Rajpurkar, Jian Zhang, Konstantin Lopyrev, and Percy Liang.
\newblock Squad: 100,000+ questions for machine comprehension of text.
\newblock \emph{arXiv preprint arXiv:1606.05250}, 2016.

\bibitem[Srivastava et~al.(2014)Srivastava, Hinton, Krizhevsky, Sutskever, and
  Salakhutdinov]{srivastava2014dropout}
Nitish Srivastava, Geoffrey Hinton, Alex Krizhevsky, Ilya Sutskever, and Ruslan
  Salakhutdinov.
\newblock Dropout: A simple way to prevent neural networks from overfitting.
\newblock \emph{The Journal of Machine Learning Research}, 15\penalty0
  (1):\penalty0 1929--1958, 2014.

\bibitem[Wang et~al.(2015)Wang, Berant, Liang, et~al.]{wang2015building}
Yushi Wang, Jonathan Berant, Percy Liang, et~al.
\newblock Building a semantic parser overnight.
\newblock In \emph{ACL (1)}, pages 1332--1342, 2015.

\bibitem[Yang et~al.(2015)Yang, Yih, and Meek]{yang2015wikiqa}
Yi~Yang, Wen-tau Yih, and Christopher Meek.
\newblock Wikiqa: A challenge dataset for open-domain question answering.
\newblock In \emph{EMNLP}, pages 2013--2018, 2015.

\bibitem[Yin et~al.(2016)Yin, Lu, Li, and Kao]{yin2016neural}
Pengcheng Yin, Zhengdong Lu, Hang Li, and Ben Kao.
\newblock Neural enquirer: learning to query tables in natural language.
\newblock In \emph{Proceedings of the Twenty-Fifth International Joint
  Conference on Artificial Intelligence}, pages 2308--2314. AAAI Press, 2016.

\bibitem[Yu et~al.(2017)Yu, Choi, Kim, Yoo, Lee, and Kim]{yu2017supervising}
Youngjae Yu, Jongwook Choi, Yeonhwa Kim, Kyung Yoo, Sang-Hun Lee, and Gunhee
  Kim.
\newblock Supervising neural attention models for video captioning by human
  gaze data.
\newblock In \emph{IEEE Conference on Computer Vision and Pattern Recognition
  (CVPR 2017). Honolulu, Hawaii}, pages 2680--29, 2017.

\bibitem[Zeiler(2012)]{zeiler2012adadelta}
Matthew~D Zeiler.
\newblock Adadelta: an adaptive learning rate method.
\newblock \emph{arXiv preprint arXiv:1212.5701}, 2012.

\bibitem[Zettlemoyer and Collins(2005)]{zettlemoyer2005learning}
Luke~S Zettlemoyer and Michael Collins.
\newblock Learning to map sentences to logical form: Structured classification
  with probabilistic categorial grammars.
\newblock In \emph{In Proceedings of the 21st Conference on Uncertainty in AI}.
  Citeseer, 2005.

\bibitem[Zhao and Mao(2017)]{zhao2017topic}
Rui Zhao and Kezhi Mao.
\newblock Topic-aware deep compositional models for sentence classification.
\newblock \emph{IEEE/ACM Transactions on Audio, Speech, and Language
  Processing}, 25\penalty0 (2):\penalty0 248--260, 2017.

\bibitem[Zhong et~al.(2017)Zhong, Xiong, and Socher]{zhongSeq2SQL2017}
Victor Zhong, Caiming Xiong, and Richard Socher.
\newblock Seq2sql: Generating structured queries from natural language using
  reinforcement learning.
\newblock \emph{CoRR}, abs/1709.00103, 2017.

\end{thebibliography}

